Structured Prediction for CRiSP Inverse Kinematics Learning with Misspecified Robot Models

With the recent advances in machine learning, problems that traditionally would require accurate modeling to be solved analytically can now be successfully approached with data-driven strategies. Among these, computing the inverse kinematics of a redundant robot arm poses a significant challenge due to the non-linear structure of the robot, the hard joint constraints and the non-invertible kinematics map. Moreover, most learning algorithms consider a completely data-driven approach, while often useful information on the structure of the robot is available and should be positively exploited. In this work, we present a simple, yet effective, approach for learning the inverse kinematics. We introduce a structured prediction algorithm that combines a data-driven strategy with the model provided by a forward kinematics function -- even when this function is misspecified -- to accurately solve the problem. The proposed approach ensures that predicted joint configurations are well within the robot's constraints. We also provide statistical guarantees on the generalization properties of our estimator as well as an empirical evaluation of its performance on trajectory reconstruction tasks.

==> algorithm.tex <==
\begin{algorithm}[h]
\SetAlgoLined
\KwResult{Write here the result }
 initialization\;
 \While{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{Self-supervised strong positives selection}
\end{algorithm}

==> macros.tex <==



%\declaretheorem[name=Theorem,numberlike=theorem]{thm}

\declaretheorem[name=Theorem,refname=Thm.]{theorem}
\declaretheorem[name=Lemma,sibling=theorem]{lemma}
\declaretheorem[name=Proposition,refname=Prop.,sibling=theorem]{proposition}
\declaretheorem[name=Remark]{remark}
\declaretheorem[name=Corollary,refname=Cor.,sibling=theorem]{corollary}
\declaretheorem[name=Definition,refname=Def.]{definition}
\declaretheorem[name=Conjecture,sibling=theorem]{conjecture}
\declaretheorem[name=Axiom]{axiom}
\declaretheorem[name=Assumption,refname=Asm.]{assumption}




\declaretheorem[name=Example]{example}



\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}


\definecolor{dgreen}{rgb}{0.00,0.49,0.00}
\definecolor{dblue}{rgb}{0,0.08,0.75}
% \usepackage{hyperref}       % hyperlinks
% \RequirePackage[colorlinks,citecolor=green,urlcolor=blue,linkcolor=blue]{hyperref}
% \hypersetup{
%     colorlinks = true,
%     citecolor=dgreen,
%     urlcolor=dblue,
%     linkcolor=dblue
% }


\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{}{}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}
\crefname{section}{Sec.}{Sec.}
\crefname{theorem}{Thm.}{Thm.}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Cor.}{Cor.}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{algorithm}{Alg.}{Algorightms}
\crefname{algocf}{Alg.}{Algorightms}

\crefname{appendix}{Appendix}{Appendices}
\crefname{subappendix}{Appendix}{Appendices}
\crefname{subsubappendix}{Appendix}{Appendices}



%------ Names & Acronyms ---------
% \newcommand{\spmlTitle}{A Structured Prediction Approach for Conditional Meta-Learning}
\newcommand{\spmlTitle}{Structured Prediction for Conditional Meta-Learning}
\newcommand{\spml}{TASML}
\newcommand{\spmlong}{Task-adaptive Structured Meta-Learning}
\newcommand{\preTrainFeat}{Pre-trained Features}
\newcommand{\lsmetal}{{\textsc{LS~Meta-Learn}}}
\newcommand{\imgnet}{\textsc{ImageNet}}
\newcommand{\mimg}{\textit{mini}\imgnet{}}
\newcommand{\timg}{\textit{tiered}\imgnet{}}
\newcommand{\cifar}{\textsc{CIFAR-FS}}
\newcommand{\leo}{{LEO}}
\newcommand{\sploss}{{\bigtriangleup}}
\newcommand{\loss}{{\bigtriangleup}}
%---------------------------------



\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}


\newcommand{\R}{{\mathbb{R}}}
\newcommand{\N}{{\mathbb{N}}}


\newcommand{\EE}{\mathbb{E}}
\newcommand{\Lagr}{\mathcal{L}}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}


\newcommand{\X}{{\mathcal{X}}}
\newcommand{\Y}{{\mathcal{Y}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\D}{{\mathcal{D}}}
\newcommand{\A}{{\mathcal{A}}}
\newcommand{\E}{{\mathcal{E}}}

\newcommand{\hh}{{\mathcal{H}}}
\newcommand{\G}{{\mathcal{G}}}

\newcommand{\hs}{{\textrm{HS}}}
\newcommand{\HS}{{\hs}}

\newcommand{\metaD}{{S}}

\newcommand{\alg}{\textrm{Alg}}
\newcommand{\jointAlg}{T}

\newcommand{\condmetapar}{\tau}
\newcommand{\Condmetapar}{{\mathcal{T}}}


\newcommand{\fhat}{\widehat{f}}

\renewcommand{\paragraph}[1]{~\newline\noindent{\bfseries #1.}}

\newcommand{\gstar}{{g^*}}


\newcommand{\eqals}[1]{\begin{align*}#1\end{align*}}

\newcommand{\eqal}[1]{\begin{align}#1\end{align}}

\renewcommand{\vec}[1]{\bm{#1}}





\newcommand{\crisp}{CRiSP}
\newcommand{\gt}{\Tilde{g}}


% \newenvironment{example}[1][]{\refstepcounter{example}\par\medskip
%   \textbf{Example~\theexample. #1} \rmfamily}{\medskip}

\newcounter{theoremdecente}[section]
\newenvironment{theoremdecente}[1][]
{\refstepcounter{theoremdecente}\par\medskip\noindent{\bfseries Theorem~\thetheoremdecente~ (#1).}\itshape}
{}


\crefname{theoremdecente}{Thm.}{Thm.}


\newenvironment{proofdecente}{\par\noindent{\itshape Proof.}}{\hfill$\square$\medskip}

==> panda_table_links.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{\small
IK performances comparison of \crisp{}-FK and SDLS on 4 desired trajectories (position and orientation) for the end-effector (EE) of a 7-DoF Panda arm.
$S$: spiral with fixed desired EE orientation;
% , with CRiSP trained on data sampled from a cube with unconstrained EE orientations
$C_0$, $C_{-\pi/4}$, $C_{+\pi/4}$: Circumference with 3 different EE orientations.
% , trained on data sampled from a solid torus surrounding the circumference.
The Panda arm's kinematic model is corrupted by introducing increasing biases (0 to 3 $deg$) at each joint.
Position (mm) and orientation (radians) root mean square errors (RMSE) are reported with their standard deviations along the trajectories.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ll|ll|ll|ll}
\multicolumn{1}{r}{\textit{}}            & \textit{Trajectory}                                 & \multicolumn{2}{c|}{\textbf{$S$}}                                       & \multicolumn{2}{c|}{\textbf{$C_0$}}                                     & \multicolumn{2}{c|}{\textbf{$C_{-\pi/4}$}}                              & \multicolumn{2}{c}{\textbf{$C_{+\pi/4}$}}\\
\cline{2-10} 
\multicolumn{1}{r}{\textit{}}            & \textit{Algorithm}                                  & \multicolumn{1}{c}{\textbf{CRiSP-FK}} & \multicolumn{1}{c|}{\textbf{SDLS}} & \multicolumn{1}{c}{\textbf{CRiSP-FK}} & \multicolumn{1}{c|}{\textbf{SDLS}} & \multicolumn{1}{c}{\textbf{CRiSP-FK}} & \multicolumn{1}{c|}{\textbf{SDLS}} & \multicolumn{1}{c}{\textbf{CRiSP-FK}} & \multicolumn{1}{c}{\textbf{SDLS}} \\ \hline
\multicolumn{1}{c|}{\textit{Bias (deg)}} & \textit{}                                           & \multicolumn{1}{c}{\textit{}}      &                                    &                                    &                                    &                                    &                                    &                                    &                                   \\
\multicolumn{1}{c|}{0}                   & \textit{}                                           & \textbf{0.739 ± 0.303}             & 1.33 ± 0.386                       & \textbf{0.602 ± 0.173}             & 0.749 ± 0.142                      & \textbf{0.548 ± 0.153}             & 0.762 ± 0.262                      & \textbf{0.576 ± 0.124}             & 3.58 ± 0.385                      \\
\multicolumn{1}{c|}{0.01}                & \textit{}                                           & \textbf{0.749 ± 0.309}             & 1.42 ± 0.393                       & \textbf{0.623 ± 0.173}             & 1.05 ± 0.141                       & \textbf{0.56 ± 0.161}              & 0.61 ± 0.208                       & \textbf{0.575 ± 0.126}             & 3.67 ± 0.388                      \\
%\multicolumn{1}{c|}{0.05}                & \textit{}                                           & \textbf{0.92 ± 0.431}              & 1.81 ± 0.392                       & \textbf{0.765 ± 0.126}             & 2.28 ± 0.139                       & \textbf{0.588 ± 0.172}             & 1.3 ± 0.03                         & \textbf{0.574 ± 0.125}             & 4.41 ± 0.154                      \\
\multicolumn{1}{c|}{0.1}                 & \textit{Pos. RMSE}                                  & \textbf{1.17 ± 0.641}              & 2.99 ± 0.294                       & \textbf{1.01 ± 0.155}              & 3.81 ± 0.141                       & \textbf{0.623 ± 0.181}             & 2.93 ± 0.05                        & \textbf{0.573 ± 0.126}             & 5.75 ± 0.165                      \\
%\multicolumn{1}{c|}{0.5}                 & \textit{(mm)}                                       & \textbf{3.75 ± 2.74}               & 14 ± 0.481                         & \textbf{3.6 ± 0.515}               & 16.1 ± 0.269                       & \textbf{1.45 ± 0.819}              & 15.9 ± 0.216                       & \textbf{0.568 ± 0.13}              & 17.1 ± 0.344                      \\
\multicolumn{1}{c|}{1}                   & \textit{}                                           & \textbf{7.31 ± 5.37}               & 27.9 ± 0.824                       & \textbf{7.26 ± 1.25}               & 31.7 ± 0.5                         & \textbf{1.8 ± 1.06}                & 32.1 ± 0.421                       & \textbf{0.56 ± 0.137}              & 35.2 ± 0.563                      \\
%\multicolumn{1}{c|}{2}                   & \textit{}                                           & \textbf{14.3 ± 10.5}               & 55.7 ± 1.61                        & \textbf{13.7 ± 2.21}               & 63.3 ± 0.959                       & \textbf{3.85 ± 2.8}                & 64.6 ± 0.818                       & \textbf{0.57 ± 0.116}              & 72.3 ± 1.03                       \\
\multicolumn{1}{c|}{3}                   & \textit{}                                           & \textbf{21.2 ± 15.5}               & 83.7 ± 2.48                        & \textbf{20.1 ± 3.44}               & 95.4 ± 1.38                        & \textbf{9.78 ± 7.95}               & 97 ± 1.2                           & \textbf{0.592 ± 0.106}             & 110 ± 1.47                        \\ \hline
\multicolumn{1}{c|}{\textit{Bias (deg)}} & \multicolumn{1}{l|}{}                               &                                    &                                    &                                    &                                    &                                    &                                    &                                    &                                   \\
\multicolumn{1}{c|}{0}                   & \textit{}                                           & 32.2 ± 19.3                        & \textbf{7.28 ± 2.29}               & 9.4 ± 0.77                         & \textbf{3.92 ± 0.95}               & \textbf{2.92 ± 0.71}               & 6.97 ± 0.11                        & \textbf{19.9 ± 1.35}               & 27.9 ± 1.03                       \\
\multicolumn{1}{c|}{0.01}                & \multicolumn{1}{l|}{}                               & 32.2 ± 19.3                        & \textbf{7.46 ± 2.19}               & 9.61 ± 0.66                        & \textbf{4.08 ± 0.48}               & \textbf{2.99 ± 0.75}               & 10 ± 0.21                          & \textbf{19.9 ± 1.35}               & 29.2 ± 1.17                       \\
%\multicolumn{1}{c|}{0.05}                & \multicolumn{1}{l|}{}                               & 35.1 ± 19.8                        & \textbf{20.9 ± 0.51}               & \textbf{12.8 ± 1.1}                & 22.4 ± 0.18                        & \textbf{3.46 ± 0.65}               & 26.9 ± 0.93                        & \textbf{19.9 ± 1.39}               & 34.6 ± 1.79                       \\
\multicolumn{1}{c|}{0.1}                 & \textit{Orn. RMSE}                                  & 40.4 ± 21.3                        & \textbf{41.2 ± 1.06}               & \textbf{20 ± 2.52}                 & 45.6 ± 0.33                        & \textbf{4.4 ± 1.45}                & 49.6 ± 1.76                        & \textbf{19.9 ± 1.41}               & 54.3 ± 1.16                       \\
%\multicolumn{1}{c|}{0.5}                 & \multicolumn{1}{l|}{\textit{(rad $\cdot 10^{-4}$)}} & \textbf{109 ± 48.3}                & 203 ± 5.8                          & \textbf{95.6 ± 8.56}               & 231 ± 1.46                         & \textbf{25.1 ± 19.3}               & 230 ± 8.4                          & \textbf{20.3 ± 1.51}               & 245 ± 2.85                        \\
\multicolumn{1}{c|}{1}                   & \multicolumn{1}{l|}{}                               & \textbf{203 ± 86.6}                & 403 ± 11.9                         & \textbf{198 ± 22.8}                & 462 ± 2.72                         & \textbf{32.8 ± 24.3}               & 453 ± 16.7                         & \textbf{21.1 ± 1.81}               & 485 ± 4.38                        \\
%\multicolumn{1}{c|}{2}                   & \multicolumn{1}{l|}{}                               & \textbf{390 ± 165}                 & 797 ± 24.7                         & \textbf{377 ± 38.9}                & 919 ± 4.84                         & \textbf{73.7 ± 57.7}               & 885 ± 33.1                         & \textbf{23.1 ± 3.15}               & 974 ± 7.82                        \\
\multicolumn{1}{c|}{3}                   & \multicolumn{1}{l|}{}                               & \textbf{611 ± 260}                 & 1.18e+03 ± 38.2                    & \textbf{548 ± 59}                  & 1.37e+03 ± 6.61                    & \textbf{189 ± 157}                 & 1.3e+03 ± 49.5                     & \textbf{25 ± 4.89}                 & 1.47e+03 ± 11.4                  
\end{tabular}%
}
\label{tab:panda_exp}
\end{table*}







